Auto-ViT-Acc: An FPGA-Aware Automatic Acceleration Framework for Vision Transformer with Mixed-Scheme Quantization

Vision transformers (ViTs) are emerging with significantly improved accuracy in computer vision tasks. However, their complex architecture and enormous computation/storage demand impose urgent needs for new hardware accelerator design methodology. This work proposes an FPGA-aware automatic ViT acceleration framework based on the proposed mixed-scheme quantization. To the best of our knowledge, this is the first FPGA-based ViT acceleration framework exploring model quantization. Compared with state-of-the-art ViT quantization work (algorithmic approach only without hardware acceleration), our quantization achieves 0.47% to 1.36% higher Top-1 accuracy under the same bit-width. Compared with the 32-bit floating-point baseline FPGA accelerator, our accelerator achieves around 5.6x improvement on the frame rate (i.e., 56.8 FPS vs. 10.0 FPS) with 0.71% accuracy drop on ImageNet dataset for DeiT-base.

==> Tables/Table_deit_scalar.tex <==
\begin{table}[htb]
\small

\caption{\textbf{Accuracy under Different Activation Scalars for DeiT-S with W4A4 Precision on ImageNet Dataset}}\label{tab:comparison_scalar}
\centering
\begin{tabular}{c c c c }%{p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
\toprule
Quantization & Actv.  & \multicolumn{2}{c}{Model Accuracy (\%)}  \\
Scheme & Scalar & Top1 & Top5\\
\hline
Baseline & - &  79.85 &  94.97 \\
Fixed (W4A4) & 10.0 &   77.41 &  93.99 \\
Fixed (W4A4) & 5.0 &  77.86 &  94.10 \\
Fixed (W4A4) & 3.0 & 78.40  & 94.38 \\
\bf{Fixed (W4A4)} & \bf{2.0}  &  \bf{78.57}  &  \bf{94.41} \\
Fixed (W4A4) & 1.0 &  78.17  & 94.09 \\
% PoT (W4A4) & max & 77.01  & 93.71  \\


\bottomrule
\end{tabular}
\end{table}
